The use of Data Augmentation as a technique for improving neural network accuracy in detecting fake news about COVID-19

This paper aims to present how the application of Natural Language Processing (NLP) and data augmentation techniques can improve the performance of a neural network for better detection of fake news in the Portuguese language. Fake news is one of the main controversies during the growth of the internet in the last decade. Verifying what is fact and what is false has proven to be a difficult task, while the dissemination of false news is much faster, which leads to the need for the creation of tools that, automated, assist in the process of verification of what is fact and what is false. In order to bring a solution, an experiment was developed with neural network using news, real and fake, which were never seen by artificial intelligence (AI). There was a significant performance in the news classification after the application of the mentioned techniques.

==> references.tex <==
@article{internetEducacao,
  title={A PANDEMIA DE COVID-19: REFLEXOS NA GARANTIA DO DIREITO {\`A} EDUCA{\c{C}}{\~A}O},
  author={de Almeida, Tha{\'\i}s Farias},
  journal={Pensar Acad{\^e}mico},
  volume={18},
  number={5},
  pages={881--894},
  year={2020}
}

@article{ding2020challenges,
  title={Challenges in Combating COVID-19 Infodemic--Data, Tools, and Ethics},
  author={Ding, Kaize and Shu, Kai and Li, Yichuan and Bhattacharjee, Amrita and Liu, Huan},
  journal={arXiv preprint arXiv:2005.13691},
  year={2020}
}

@article{madani2021using,
  title={Using artificial intelligence techniques for detecting Covid-19 epidemic fake news in Moroccan tweets},
  author={Madani, Youness and Erritali, Mohammed and Bouikhalene, Belaid},
  journal={Results in Physics},
  pages={104266},
  year={2021},
  publisher={Elsevier}
}

@article{patwa2020fighting,
  title={Fighting an infodemic: Covid-19 fake news dataset},
  author={Patwa, Parth and Sharma, Shivam and PYKL, Srinivas and Guptha, Vineeth and Kumari, Gitanjali and Akhtar, Md Shad and Ekbal, Asif and Das, Amitava and Chakraborty, Tanmoy},
  journal={arXiv preprint arXiv:2011.03327},
  year={2020}
}

@article{mookdarsanit2021covid,
  title={The COVID-19 fake news detection in Thai social texts},
  author={Mookdarsanit, Pakpoom and Mookdarsanit, Lawankorn},
  journal={Bulletin of Electrical Engineering and Informatics},
  volume={10},
  number={2},
  pages={988--998},
  year={2021}
}

@incollection{kalsnes2018fake,
  title={Fake news},
  author={Kalsnes, Bente},
  booktitle={Oxford Research Encyclopedia of Communication},
  year={2018}
}

@article{pereira2021desinformaccao,
  title={A desinforma{\c{c}}{\~a}o como estrat{\'e}gia pol{\'\i}tica: uma an{\'a}lise dos tweets de ataque {\`a} imprensa postados por Jair Messias Bolsonaro no ano de 2019},
  author={Pereira, Matheus Ribeiro},
  journal={Aquila},
  number={24},
  pages={97--110},
  year={2021}
}

@article{dias2019towards,
  title={Towards fake news detection in Portuguese: New dataset and a claim-based approach for automated detection},
  author={Dias, Cristiano Ruschel Marques},
  year={2019}
}

@MISC{FacebookFakeNewsTool,
  title = {"Facebook Messenger ganha novas ferramentas para combater assédio e fake news"},
  howpublished = {\url{https://tinyurl.com/ferramentatwitterfacebook}},
  note = {Accessed: 2021-05-23},
  author = {CanalTech},
  year = {2021}
}

@MISC{LATAMcoronavirus,
  title = {LATAM Coronavírus},
  howpublished = {\url{https://chequeado.com/latamcoronavirusportugues/}},
  note = {Accessed: 2021-05-22},
  author = {Chequeado},
  year = {2021}
}

@misc{TwitterFakeNewsTool,
  title = {Twitter testa nova ferramenta para conter desinformação e fake news},
  howpublished = {\url{https://tinyurl.com/ferramentamessenger}},
  note = {Accessed: 2021-05-23},
  author = {CanalTech},
  year = {2020}
}


@misc{Fake.Br,
  title = {Fake.Br Corpus},
  howpublished = {\url{https://github.com/roneysco/Fake.br-Corpus}},
  note = {Accessed: 2021-05-19},
  author = {Roney Santos},
  year = {2021}
}

@misc{Collins2020,
  title = {Collins Dictionary 2020},
  howpublished = {\url{https://www.collinsdictionary.com/woty}},
  note = {Accessed: 2021-05-15},
  author = {Collins},
  year = {2020}
}

@misc{Lupa2020,
  title = {Lupa, a primeira agência fact-checking do Brasil},
  howpublished = {\url{https://piaui.folha.uol.com.br/lupa/?utm_source=Search&utm_medium=cpc&utm_campaign=lupa5anos}},
  note = {Accessed: 2021-05-16},
  author = {Folha},
  year = {2021}
}

@article{neto2020fake,
  title={Fake news no cen{\'a}rio da pandemia de Covid-19},
  author={Neto, Mercedes and de Oliveira Gomes, Tatiana and Porto, Fernando Rocha and Rafael, Ricardo de Mattos Russo and Fonseca, Mary Hellem Silva and Nascimento, Julia},
  journal={Cogitare Enfermagem},
  volume={25},
  year={2020}
}

@article{DBLP:journals/corr/abs-1810-04805,
  author    = {Jacob Devlin and
               Ming{-}Wei Chang and
               Kenton Lee and
               Kristina Toutanova},
  title     = {{BERT:} Pre-training of Deep Bidirectional Transformers for Language
               Understanding},
  journal   = {CoRR},
  volume    = {abs/1810.04805},
  year      = {2018},
  url       = {http://arxiv.org/abs/1810.04805},
  archivePrefix = {arXiv},
  eprint    = {1810.04805},
  timestamp = {Tue, 30 Oct 2018 20:39:56 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1810-04805.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{singh2020fake,
  title={Fake News Detection: a comparison between available Deep Learning techniques in vector space},
  author={Singh, Lovedeep},
  booktitle={2020 IEEE 4th Conference on Information \& Communication Technology (CICT)},
  pages={1--4},
  year={2020},
  organization={IEEE}
}

@article{shushkevich2021tudublin,
  title={TUDublin team at Constraint@ AAAI2021--COVID19 Fake News Detection},
  author={Shushkevich, Elena and Cardiff, John},
  journal={arXiv preprint arXiv:2101.05701},
  year={2021}
}

@article{gupta2021hostility,
  title={Hostility Detection and Covid-19 Fake News Detection in Social Media},
  author={Gupta, Ayush and Sukumaran, Rohan and John, Kevin and Teki, Sundeep},
  journal={arXiv preprint arXiv:2101.05953},
  year={2021}
}

@article{paka2021cross,
  title={Cross-SEAN: A cross-stitch semi-supervised neural attention model for COVID-19 fake news detection},
  author={Paka, William Scott and Bansal, Rachit and Kaushik, Abhay and Sengupta, Shubhashis and Chakraborty, Tanmoy},
  journal={Applied Soft Computing},
  pages={107393},
  year={2021},
  publisher={Elsevier}
}

@article{panis2016overview,
  title={Overview of research on facial ageing using the FG-NET ageing database},
  author={Panis, Gabriel and Lanitis, Andreas and Tsapatsoulis, Nicholas and Cootes, Timothy F},
  journal={Iet Biometrics},
  volume={5},
  number={2},
  pages={37--46},
  year={2016},
  publisher={IET}
}

@MISC {python,
    author = "PYTHON",
    title  = "PYTHON",
    url    = "www.python.org/about",
    year={2021}
}

@MISC {cientistadedados,
    author = "INSIGHTLAB UFC",
    title  = "Pythonx na área de Data Science",
    note="{Disponível em: \url{https://tinyurl.com/linguagemdatascience}}",
    year={2021}
}

@MISC {NLP,
    author = "NLP",
    title  = "NLP",
    note="{Disponível em: \url{https://www.nlp.com/what-is-nlp/}}",
    year={2021}
}

https://research.google/teams/language/

@MISC {googlenlp,
    author = "Google",
    title  = "Google Research",
    note="{Disponível em: \url{https://research.google/teams/language/}}",
    year={2021}
}

@MISC {neuralnetowrk,
    author = "Stanford",
    title  = "História da Rede Neural",
    note="{Disponível em: \url{https://cs.stanford.edu/people/eroberts/courses/soco/projects/neural-networks/History/history1.html}}",
    year={2021}
}

@MISC {ibmdataset,
    author = "IBM",
    title  = "Dataset",
    note="{Disponível em: \url{https://www.ibm.com/docs/en/zos-basic-skills?topic=more-what-is-data-set}}",
    year={2021}
}

@MISC {pydictionary,
    author = "PyPi",
    title  = "PyDictionary",
    note="{Disponível em: \url{https://pypi.org/project/PyDictionary/}}",
    year={2021}
}

@MISC {tensorflow,
    author = "TensorFlow",
    title  = "TensorFlow",
    note="{Disponível em: \url{https://www.tensorflow.org/tutorials/images/data_augmentation}}",
    year={2021}
}

@MISC {nltk,
    author = "NLTK",
    title  = "Tokenize",
    note="{Disponível em: \url{http://nltk.sourceforge.net/doc/pt-br/tokenize.html}}",
    year={2021}
}

@MISC {SpaCy,
    author = "PyPi",
    title  = "SpaCy",
    note="{Disponível em: \url{https://pypi.org/project/SpaCy/}}",
    year={2021}
}

@MISC {singularity014,
    author = "singularity014",
    title  = "Singularity014 - Autor do Projeto Base",
    note="{Disponível em: \url{
https://github.com/singularity014/BERT_FakeNews_Detection_Challenge}}",
    year={2021}
}






